Extension of ACETONE C code generator for multi-core architectures

As the industry's interest in machine learning has grown in recent years, some solutions have emerged to safely embed them in safety-critical systems, such as the C code generator ACETONE. However, this framework is limited to generating sequential code, which cannot make most of the multi-core architectures. In this paper, we initiate an extension of ACETONE for the generation of parallel code by formally defining our processor assignment problem and surveying the state of the art on existing solutions. In the final paper, we will introduce the completed extension, including the implementation of the scheduling heuristic, the creation of templates implementing synchronization mechanisms, and an evaluation of the worst-case execution time of the framework's layers.

==> reviews.tex <==
SUBMISSION: 55
TITLE: Extension of ACETONE C code generator for multi-core architectures

-------------------------  METAREVIEW  ------------------------
RECOMMENDATION: accept
TEXT:
All reviewers appreciate the clear presentation of the approach and the technical soundness of your work.

One major concern among many reviewers is that you need to better explain, and justify with experimental results, your design choices. In particular:

* Why choose a parallelization method for neural networks that is more complex than standard multi-core solutions for computing convolutions, based on parallel computation of each layer ?

* How do you support your claim that your approach generates code that is easier to certify for embedded, safety-critical systems.


----------------------- REVIEW 1 ---------------------

SUBMISSION: 55
TITLE: Extension of ACETONE C code generator for multi-core architectures
AUTHORS: Yanis Aït-Aïssa, Thomas Carle, Benjamin Lesage and Claire Pagetti

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----------- Reviewer's confidence -----------
SCORE: 5 ((expert))
----------- Relevance to ERTS -----------
SCORE: 2 (poor)
----------- Originality/Novelty -----------
SCORE: 2 (poor)
----------- Positioning wrt the state of the art -----------
SCORE: 4 (good)
----------- Quality of the presentation -----------
SCORE: 4 (good)
----------- Technical soudness -----------
SCORE: 4 (good)
----------- Review -----------
* Summary
The authors describe how to extend the ACETONE C to multi-core microcontrollers.

* Main strengths/weaknesses:
I have huge issues with the paper. My main concern is actually stated by the authors themselves in Section 4:
"Indeed the operation behing some layers, such as the convolution layer, can be divided into smaller operations, increasing the number of tasks to be scheduled"
That is correct. All layers in neural networks, that typically contribute the vast majority of runtime, like convolutions, fully connected layers, LSTMs, GRU, are based on matrix multiplications and similar algorithms.
These algorithms have existing, good solutions to parallelize them on multi-core machines.
Why do I then need a much much more complicated algorithm to parallelize over layers?
Especially because such an approach can only work for non-sequential models.
However, sequential models are very often used on smaller hardware.

The authors state in 1.1 that
"the generated code is designed to be easily certifiable for being embedded in aeronautical safety-critical systems".
I would like to get some details on what this means compared to the code generated by other tools like the Matlab Embedded Coder or those in the ML Perf Tiny benchmark
https://mlcommons.org/working-groups/benchmarks/tiny/
that produce C code as well or use library implementations.

But, having functional safety in mind, it appears logical to use as simple a technique to reach multi-core parallelization as possible, i.e., parallelization per-layer.
Especially because I do not expect substantial further performance benefits from the much more complicated technique that the authors describe.

** Relevance:

        Relevant for ERTS
** Approach/methods:
        See main strengths and weaknesses

** Technical soundness:
        The paper gives no reason why the approach should provide a benefit over simple per-layer parallelization.

** Positioning:

** Quality of the presentation:
The paper is written in good-quality English.

* Detailed Comments:
----------- Ways of improvement for the shepherding process -----------
A strong argument for the much more complex approach that the authors propose for the parallelization of neural networks would make the paper a useful contribution.


----------------------- REVIEW 2 ---------------------

SUBMISSION: 55
TITLE: Extension of ACETONE C code generator for multi-core architectures
AUTHORS: Yanis Aït-Aïssa, Thomas Carle, Benjamin Lesage and Claire Pagetti

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----------- Reviewer's confidence -----------
SCORE: 4 ((high))
----------- Relevance to ERTS -----------
SCORE: 5 (excellent)
----------- Originality/Novelty -----------
SCORE: 4 (good)
----------- Positioning wrt the state of the art -----------
SCORE: 4 (good)
----------- Quality of the presentation -----------
SCORE: 4 (good)
----------- Technical soudness -----------
SCORE: 4 (good)
----------- Review -----------
The authors present the implementation and inference of deep neural networks (DNN) on multi-core architectures for safety-critical avionics applications. This is an important and timely problem, where real-time constraints and certification challenges hinder straightforward deployment. The motivation is well positioned: while dedicated accelerators are not yet widely certifiable, industry is transitioning from single-core to multi-core architectures, creating the need for efficient, predictable, and certifiable code generation tools.

The authors build on the ACETONE framework, which already ensures sequential C-code generation with analyzable timing properties, and propose extending it to multi-core execution. The methodology is grounded in directed acyclic graph (DAG) modeling of DNNs, and the scheduling problem is clearly formalized. The state of the art is reviewed adequately, though the discussion of ILP scalability is acknowledged as incomplete and deferred to the final version.

The future experimental plan is realistic and strengthens the applicability of the work. However, the current draft lacks concrete evaluation: no testing protocol or preliminary results are presented, making it difficult to assess performance gains or certification-readiness.
----------- Ways of improvement for the shepherding process -----------
- validation of scheduling heuristics against baselines


----------------------- REVIEW 3 ---------------------

SUBMISSION: 55
TITLE: Extension of ACETONE C code generator for multi-core architectures
AUTHORS: Yanis Aït-Aïssa, Thomas Carle, Benjamin Lesage and Claire Pagetti

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----------- Reviewer's confidence -----------
SCORE: 4 ((high))
----------- Relevance to ERTS -----------
SCORE: 5 (excellent)
----------- Originality/Novelty -----------
SCORE: 5 (excellent)
----------- Positioning wrt the state of the art -----------
SCORE: 4 (good)
----------- Quality of the presentation -----------
SCORE: 5 (excellent)
----------- Technical soudness -----------
SCORE: 5 (excellent)
----------- Review -----------
ACETONE-C is a framework for the analysis and code generation targeting the implementation of neural networks on multicore embedded systems. Its goals include to simplify certification of the end results and perform precise timing analysis, in cases where there are no integrated accelerators.

The paper extends previous works on the ACETONE-C compiler, which only generated sequential C code, for a single core, by allowing concurrent execution on a system of parallel, real-time tasks.

The short abstract is very clear, well organised and provides an extensive state of the art on ILP based methods for optimising the scheduling of the resulting code.

Strengths:

- Important and timely subject, in scope with the  main topics of ERTS.

- Automatic parallelization of code is a difficult problem and the work addresses issues that are not often taken into account in other approaches, such as predictability of WCET and certifiability of the generated code.

- It is a substantial improvement on a previous work, which was already quite significant. The authors plan to include a detailed experimental evaluation and benchmarks on an actual processor in the long version of the paper.


Weaknesses:

- You need to better justify some of your core design choices. Especially, why do you choose to parallelize at the task level instead of using a simpler approach based on parallel computation of layers ?

- There are several strong assumptions about design choices which makes the approach difficult to generalize and suitable for only a limited list of processors.

- Some choices lack explanation and motivations: it assumes a uniform memory access model, it does not address caching issues (no mention of cache hierarchies or interferences for concurrent memory accesses), no preemption, there is no information about how operations are partitioned into tasks  and how the granularity is chosen.
----------- Ways of improvement for the shepherding process -----------
There is a large body of work on automatic optimization and parallelization of programs that compute convolutions, or that contain nested loops. There are other approaches than ILP-based scheduling that could be worth mentioning, Some examples that come to mind are the polyhedral compilation model (see for instance the work of Baghdadi on the TIRAMISU compiler), or systolic-based design techniques, based on optimized pipelining and data-flows between instructions. Could you comment on whether these approaches are amenable to implementation using real-time tasks.


----------------------- REVIEW 4 ---------------------

SUBMISSION: 55
TITLE: Extension of ACETONE C code generator for multi-core architectures
AUTHORS: Yanis Aït-Aïssa, Thomas Carle, Benjamin Lesage and Claire Pagetti

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
The abstract provides a good bibliography and hints at promising details. The modelization is sound and the 2 main contributions are identified (modification of ACETONE and impact on WCET). However major work for these contributions is still to be done, it would have been relevant to add more details on these tasks - transforming a weak accept into an accept.
----------- Reviewer's confidence -----------
SCORE: 4 ((high))
----------- Relevance to ERTS -----------
SCORE: 5 (excellent)
----------- Originality/Novelty -----------
SCORE: 4 (good)
----------- Positioning wrt the state of the art -----------
SCORE: 5 (excellent)
----------- Quality of the presentation -----------
SCORE: 4 (good)
----------- Technical soudness -----------
SCORE: 5 (excellent)
----------- Review -----------
The abstract presents the problem of scheduling efficiently Deep Neural Network computation on a multi-core platform, especially with warranties on output precision regarding numerical error and Worst Case Execution Time bounds. The authors present a modalization of the problem in the form of a Directed Acyclic Graph, which allows to express the problem as an optimization problem for minimizing the total time. The author provide a review of three classes of methods to schedule the node of the graph - either an exact ILM-based method, a set of heuristics or a search approach benefiting from the tree structure.

The abstract is well written and the bibilography is relevant. The abstract cuts a bit short : the authors explain that they intend in the full paper to develop three parts : (1) the scalability of the heuristics, (2) the extension of ACETONE with synchronization mecanisms and repartition on multiple nodes, and (3) experimental and analytical computation of WCET.

Note that ACETONE is not sufficiently described in the abstract to understand the changes that will need to be done to move from mono to multi core - the final paper should be articulated around it because it seems to be the main novel contribution. The second missing point is to explain how the WCET can be computed with the planned extension - which will necessitate both a theoretical work and experimental proof.
----------- Ways of improvement for the shepherding process -----------
Rework the introduction with strong positionning of your work from the bibliography : at the moment most of the description of your novel work is hinted in the conclusion. You should state clearly what you add to the state of the art.

Be sure to detail which warranties remain true when going from monocore to multicore : semantic preservation, bounds on numerical error in the output, WCET,...

The current modelization is sound, but be clear if (and how) it wors with different types of DNN : recurrent NN, Encoder/ Decoder, architectures with randomness such as dropout layers.


